CrossCLR: Cross-modal Contrastive Learning For Multi-modal Video Representations

Contrastive learning allows us to flexibly define powerful losses by contrasting positive pairs from sets of negative samples. Recently, the principle has also been used to learn cross-modal embeddings for video and text, yet without exploiting its full potential. In particular, previous losses do not take the intra-modality similarities into account, which leads to inefficient embeddings, as the same content is mapped to multiple points in the embedding space. With CrossCLR, we present a contrastive loss that fixes this issue. Moreover, we define sets of highly related samples in terms of their input embeddings and exclude them from the negative samples to avoid issues with false negatives. We show that these principles consistently improve the quality of the learned embeddings. The joint embeddings learned with CrossCLR extend the state of the art in video-text retrieval on Youcook2 and LSMDC datasets and in video captioning on Youcook2 dataset by a large margin. We also demonstrate the generality of the concept by learning improved joint embeddings for other pairs of modalities.

==> sections/crossclr_code.tex <==
\begin{algorithm}[t]
    \caption{Pseudocode of CrossCLR in a PyTorch style.}
    \label{alg:code}
    {\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{mm}: matrix multiplication; \texttt{cat}: concatenation.
    %\vspace{-1.em}
    }
    
    \definecolor{codeblue}{rgb}{0.35,0.4,0.7}
    \lstset{
      backgroundcolor=\color{white},
      basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
      columns=fullflexible,
      breaklines=true,
      captionpos=b,
      commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
      keywordstyle=\fontsize{7.2pt}{7.2pt},
    %  frame=tb,
    }
    \begin{lstlisting}[language=python]
    # enc_v, enc_t: encoder networks for video and text
    # in_v, in_t: input video and text embeddings (BxD)
    # t: temperature, n_keep: 1-(pruning_percentage)
    # t_w: loss weightening temperature
    # mask = 1-np.eye(B)
    # def norm_w(x): return x/sum(x)
    # def mean_w(x,w,t): return sum(x)/(sum(exp(w/t)))
    
    # Encode input video and text embeddings
    emb_v, emb_t = enc_v(in_v), enc_t(in_t)   
 
    # Compute positive and negative logits
    l_vt = mm(emb_v,emb_t.t())/t  #video to text
    l_tv = mm(emb_t,emb_v.t())/t #text to video
    l_vv = (mm(emb_v,emb_v.t())/t)*mask #video to video
    l_tt = (mm(emb_t,emb_t.t()/t)*mask #text to text
 
    # Compute proximity of semantics
    prox_vid = mean(mm(in_v, in_v.t()) * mask) 
    prox_txt = mean(mm(in_t, in_t.t()) * mask) 
    scores_v, ind_v = sort(prox_vid)       
    scores_t, ind_t = sort(prox_txt)  
 
    # Prune negative samples
    l_vv_p = l_vv[:, ind_v[:n_keep]]   
    l_tt_p = l_tt[:, ind_t[:n_keep]]  
 
    # Concatenate positive and negative logits
    l_vtv = cat([l_vt, t_w * l_vv_p], dim=1)    
    l_tvt = cat([l_tv, t_w * l_tt_p], dim=1)
    
    # Calculate the loss 
    labels = arange(l_vt.shape[0])   
    loss_vtv = cross_entropy_loss(l_vtv, labels)
    loss_tvt = cross_entropy_loss(l_tvt, labels)
 
    # Weight losses based on semantic proximity 
    w_vtv = norm_w(prox_vid)
    w_tvt = norm_w(prox_vid)
    loss_vtv = loss_vtv * exp(w_vtv / t_w) 
    loss_tvt = loss_tvt * exp(w_tvt / t_w) 
 
    loss = (mean_w(loss_vtv, w_vtv, t_w) +
              mean_w(loss_tvt, w_tvt, t_w) ) /2
 
    \end{lstlisting}
 \end{algorithm}
